Tunneling of quasiholes in the fractional quantum Hall regime

The elementary low energy excitations in the fractional quantum Hall (FQH) regime are known to be fractionally charged quasiparticles and quasiholes. This work focusses on quasiholes in a finite system of a few electrons treated by exact numerical diagonalization. Recent experimental [Chung et al., PRB 67, 201104 (2003)] and theoretical [Kane, Fisher, PRB 67, 045307 (2003)] work on quantum point contacts in the FQH regime showed strong evidence for single quasiparticle tunneling to be forbidden at low temperature. We want to gain insight into such constricted FQH systems by a numerical approach. Initially the basics of numerically treating a system in rectangular geometry and procedures to insert a quasihole excitation are presented. The excitations' stability and fractional charge is confirmed for different interactions. The question of quasihole tunneling is approached in two different systems: 1. A system posessing bound, localized states of a quasihole shows evidence for tunnel coupling between these states to exist. 2. Different potential forms to model a quantum point contact are investigated and the injection of a single quasihole near the constriction is surveyed in the system's time evolution.

==> theory/fraccharge.tex <==
\subsection{Numerical results for fractionally-charged excitations}
By applying the operator for creating a quasihole derived in section \ref{sec:QuasiHoles} on one of the degenerate ground states of a homogeneous system one obtains a wavefunction in a system with one additional flux quantum.
After creting this wavefunction any observable can be evaluated. Here we will focus on the electronic density
$\rho(\vec r) = \int_\Omega \; d\vec r_1 \ldots d\vec r_{N_e-1} |\Psi(\vec r_1,...,r_{N_e-1}, \vec r)|^2$, where $\Omega$ is the domain of the unit cell.
On review of equation (\ref{eq:HoleEx}) the wavefunction vanishes whenever one of the electrons' coordinates approaches the point where the hole was inserted. Thus it is expected to see a dip in the density in the vicinity of the quasi hole. This is confirmed by the numerical calculation. 

Here the operator was applyed to a system with 5 electrons and 15 flux quanta giving a filling factor of $\nu = \frac{1}{3}$.
The resuting density (coloured surface) is shown in figure (\ref{fig:FracCharge}). Additionally a gaussian shaped fit was drawn in the same figure. 
The area below this peak is $2 \pi l_0^2$ which is the area per flux quantum (see equation \ref{eq:FluxCondition}). In the homogeneous system there is a charge of $q_{fq} = e\frac{N_e}{N_s} = e \nu$ in this area.
The comparision of the two curves shows that the charge $q_{qh}$ which was repulsed from the hole is approximately of the same size $q_{qh} \simeq q_{fq} = e\nu$.
\begin{figure}[htbp]
  \includegraphics{pictures/fraccharge.eps}
  \caption{Electronic density of a quasihole-state}
  \label{fig:FracCharge}
\end{figure}




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

